Numerical Optimizations for Weighted Low-rank Estimation on Language Model

Singular value decomposition (SVD) is one of the most popular compression methods that approximate a target matrix with smaller matrices. However, standard SVD treats the parameters within the matrix with equal importance, which is a simple but unrealistic assumption. The parameters of a trained neural network model may affect task performance unevenly, which suggests non-equal importance among the parameters. Compared to SVD, the decomposition method aware of parameter importance is the more practical choice in real cases. Unlike standard SVD, weighted value decomposition is a non-convex optimization problem that lacks a closed-form solution. We systematically investigated multiple optimization strategies to tackle the problem and examined our method by compressing Transformer-based language models. Further, we designed a metric to predict when the SVD may introduce a significant performance drop, for which our method can be a rescue strategy. The extensive evaluations demonstrate that our method can perform better than current SOTA methods in compressing Transformer-based language models.

==> ACL2022_relatedWork.tex <==
\section{Related Work}

==> tab_fig/SVD-block.tex <==
\begin{figure*} [htbp]
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[height=4.1cm]{fig/SVD-qkv-ao.pdf}
       \caption{SVD performance on  768 $\times$ 768 dimension matrix
       %: Query, Key, Value, and Attention\_out
       }
       \label{fig:svd-sub-structure:qkv-ao}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\includegraphics[height=4.1cm]{fig/SVD-id-o.pdf}
\centering
       \caption{SVD performance on  3072 $\times$ 768 dimension matrix
       %: Intermediate and Output
       }
   \label{fig:svd-sub-structure:id-o}
\end{subfigure}
\caption{The performance of SVD on the STSB task, when only factorizing a particular type of  sub-structures (Key, Query, Value, Attention, Intermediate, or Output).
The red dash line denotes the original performance. 
%The numbers are metric $\varphi ({\bf{W}})$ calculated by Equation (\ref{equ:var}).
%The values of $\varphi ({\bf{W}})$ can well predict the performance of SVD, that matrix with a larger $\varphi ({\bf{W}})$ will always end up with a larger performance drop after applying SVD.
%Especially, the performance changes of Query and Key sub-structure are almost identical, and their  $\varphi ({\bf{W}})$ are extremely close (1.16E-03 for Query and 1.17E-03 for Key). 
}
\label{fig:svd-sub-structure}
\end{figure*}

==> tab_fig/TWSVD-block.tex <==
\begin{figure*} [htbp]
  \begin{subfigure}[b]{.49\textwidth}
   \centering
   \includegraphics[height=4.1cm]{fig/TWSVD-qkv-ao.pdf}
       \caption{FVD performance on  768 $\times$ 768 dimension matrix
       %: Query, Key, Value, and Attention\_out
       }
       \label{fig:fvd-sub-structure:qkv-ao}
       \end{subfigure}
\begin{subfigure}[b]{.49\textwidth}
\centering
\includegraphics[height=4.1cm]{fig/TWSVD-id-o.pdf}
       \caption{FVD performance on  3072 $\times$ 768 dimension matrix
       %: Intermediate and Output
       }
   \label{fig:fvd-sub-structure:id-o}
\end{subfigure}
\caption{The performance of FVD on the STSB task, when only factorizing a particular type of  sub-structures (Key, Query, Value, Attention, Intermediate, or Output) in Transformer blocks.
}
\label{fig:fvd-sub-structure}
\end{figure*}

==> tab_fig/tab1.tex <==

\begin{table*}%[!tbp]
\centering
\caption{Results of CoNLL and GLUE benchmark. G-Avg means the average of GLUE tasks, A-Avg denotes the average of all tasks, including CoNLL.
Our FVD with 66.5M parameters is the best performer in terms of both average scores. 
}
\label{tab:GLUE}
\renewcommand\tabcolsep{2.0pt}
\resizebox{1\textwidth}{!}{
\begin{tabular}
%{p{2.3cm}|c|p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}p{0.7cm}|p{0.7cm}}
{|l|l|c|ccccccc|c|c|c|}
\toprule
Task & #Param & CoNLL & CoLA & MNLI & MRPC & QNLI & QQP & SST-2 & STSB & G-Avg & A-Avg \\\midrule
Bert$\_{base}$ & 109.5M & 94.82 & 55.72 & 84.68 & 88.62 & 91.45 & 87.85 & 92.89 & 88.45 & 84.24 & 85.56 \\\midrule
distilBERT & 67.0M & 93.96 & 49.75 & 82.04 & 88.73 & 89.33 & 86.71 & 90.37 & 86.13 & 81.87 & 83.38 \\
MiniLM & 67.0M & 93.20 & 43.31 & 83.84 & 89.05 & 90.55 & 86.70 & 91.40 & 88.11 & 81.85 & 83.27 \\
TinyBERT6 & 67.0M & 93.15 & 41.24 & 83.82 & 90.55 & 90.59 & 86.94 & 92.09 & 89.41 & 82.09 & 83.47 \\\midrule
FVD & 66.5M & 94.15 & 52.17 & 83.41 & 89.00 & 90.33 & 86.85 & 91.06 & 88.49 & \bf{83.05} & \bf{84.43} \\
w/o finetune & 66.5M & 86.26 & 20.57 & 70.65 & 79.62 & 64.42 & 76.00 & 87.73 & 68.98 & 66.85 & 69.28 \\
SVD & 66.5M & 94.03 & 42.67 & 82.66 & 86.60 & 89.64 & 87.44 & 91.06 & 86.80 & 80.98 & 82.61 \\
w/o finetune & 66.5M & 39.30 & 1.73 & 35.48 & 63.84 & 38.24 & 60.02 & 75.80 & 23.10 & 42.6 & 42.19 \\\midrule
FVD & 49.9M & 93.51 & 39.34 & 82.15 & 88.27 & 88.81 & 87.03 & 89.9 & 86.96 & 80.35 & 82.00 \\
w/o finetune & 49.9M & 5.95 & 57.01 & 55.27 & 30.25 & 49.59 & 60.81 & 79.13 & 53.72 & 55.11 & 48.97 \\
SVD & 49.9M & 92.80 & 19.33 & 81.05 & 81.97 & 86.56 & 86.87 & 89.22 & 80.61 & 75.09 & 77.30 \\
w/o finetune & 49.9M & 2.74 & 0.22 & 37.00 & 0.00 & 49.46 & 36.94 & 58.26 & 16.51 & 28.34 & 25.14 \\\midrule
FVD & 37.2M & 91.88 & 21.43 & 79.06 & 85.04 & 84.33 & 85.95 & 88.99 & 85.97 & 75.82 & 77.83 \\
w/o finetune & 37.2M & 11.55 & 4.50 & 35.76 & 0.00 & 49.46 & 55.06 & 72.71 & 32.80 & 35.76 & 32.73 \\
SVD & 37.2M & 90.42 & 13.76 & 78.00 & 81.95 & 79.57 & 84.11 & 87.50 & 58.67 & 69.08 & 71.75 \\
w/o finetune & 37.2M & 2.16 & 0.00 & 32.54 & 0.00 & 49.46 & 3.44 & 51.38 & 5.45 & 20.32 & 18.05 \\
\bottomrule
\end{tabular}
}
\end{table*}


